PlaceIT: Placement-based Inter-Chiplet Interconnect Topologies

2.5D integration technology is gaining traction as it copes with the exponentially growing design cost of modern integrated circuits. A crucial part of a 2.5D stacked chip is a low-latency and high-throughput inter-chiplet interconnect (ICI). Two major factors affecting the latency and throughput are the topology of links between chiplets and the chiplet placement. In this work, we present PlaceIT, a novel methodology to jointly optimize the ICI topology and the chiplet placement. While state-of-the-art methods optimize the chiplet placement for a predetermined ICI topology, or they select one topology out of a set of candidates, we generate a completely new topology for each placement. Our process of inferring placement-based ICI topologies connects chiplets that are in close proximity to each other, making it particularly attractive for chips with silicon bridges or passive silicon interposers with severely limited link lengths. We provide an open-source implementation of our method that optimizes the placement of homogeneously or heterogeneously shaped chiplets and the ICI topology connecting them for a user-defined mix of four different traffic types. We evaluate our methodology using synthetic traffic and traces, and we compare our results to a 2D mesh baseline. PlaceIT reduces the latency of synthetic L1-to-L2 and L2-to-memory traffic, the two most important types for cache coherency traffic, by up to 28% and 62%, respectively. It also achieve an average packet latency reduction of up to 18% on traffic traces. PlaceIT enables the construction of 2.5D stacked chips with low-latency ICIs.

==> 11_optimization_algorithms.tex <==
\section{Details on Optimization Algorithms}
\label{app:opt}


In this section, we provide details on the optimization algorithms used in this work.
To illustrate these algorithms, we apply them to the following example problem:

\begin{center}
\textit{Given a blackbox cost function $f:[0,1]^3 \to \mathbb{R}$, find\\values for $a,b,c \in [0,1]$ such that $f(a,b,c)$ is minimized.}
\end{center}

\ps{Introduce "Best Random" as a baseline}

\subsection{Best Random}
\label{app:opt-br}

A na\"ive optimization algorithm is to generate many sets of random numbers $a,b,c \in [0,1]$ and to evaluate the cost function $f(a,b,c)$ for all of them.
We keep track of the values of $a,b,$ and $c$ that yield the lowest cost $f(a,b,c)$.
We use this na\"ive algorithm to verify that our more elaborate optimization algorithm perform better than random.
\Cref{alg:best-random} shows the pseudocode of the \gls{br} algorithm.

\input{alg_best_random.tex}

\ps{Explain the Genetic Algorithm}

\subsection{The Genetic Algorithm}
\label{app:opt-ga}

The \gls{ga} mimics biological evolution to solve an optimization problem.
We start with a randomly generated population of $P$ individuals.
An individual is one solution to our optimization problem, in our example, an individual is a set of numbers $a,b,c \in [0,1]$.
The algorithm iterates through generations of individuals, where each generation is formed based on the previous generation.
There are many strategies to form the next generation, in \name, we use the following policy:
The $E$ individuals of the current population that exhibit the lowest cost proceed to the next generation (elitism selection \cite{ga-elite}).

\input{tab_background_ga}

The remaining $(P-E)$ free spots in the next generation are filled with newly generated individuals called children.
A child is created by merging two parent-individuals of the current generation (crossover).
In our example, a crossover could mean that for each of the child's variables $a,b,$ and $c$, we randomly decide whether to adopt the value from the first or from the second parent.
Many methods of selecting parents exist \cite{ga-1}.
In our work, we use the tournament selection method \cite{ga-tourn} where for each child, we repeat the following process two times:
Select $T$ individuals of the current population u.a.r. 
Out of these $T$ individuals, select the one with the lowest cost function as a parent.
In the unlikely case that the same individual is selected as both parents, repeat the process until two unique parents are found.
When a child is created, there is a probability $p_m$ that it experiences a mutation.
In our example, a mutation could mean that we increase/decrease the value of one of the three variables by a random amount.
In the end, we report the lowest-cost individual as our solution.
\Cref{tab:back-ga} lists the parameters of the \gls{ga} and \Cref{alg:genetic-algorithm} provides its pseudocode.

\input{alg_genetic_algorithm.tex}

\ps{Explain Simulated Annealing}

\subsection{Simulated Annealing}
\label{app:opt-sa}

Simulated annealing is an optimization algorithm that is based on the annealing process in which a material is heated up and cooled down slowly in order to alter its properties.
At the beginning, we generate a random solution to our problem.
In our example, this corresponds to assigning random values to the variables $a,b,$ and $c$.
In each iteration of the algorithm, we create a slight modification of the current solution.
In our example, we could increase or decrease one of the three variable by a random amount.
If this new solution has a lower cost than our current solution, then we accept it, i.e., we take it as our current solution.
If the new solution has a higher cost than our current solution, then, we only accept it with a certain probability $p$. 
This probability changes over the course of the execution, which is where the magic of simulated annealing lies.
The probability $p$ is computed based on the Metropolis criterion \cite{metropolis}:


\begin{equation} \label{eq:back-opt-metro}
	p = e^{-\Delta / T}
\end{equation}

Here, $\Delta$ is the difference between the cost of the new solution and the cost of the current solution, and $T$ is the current temperature of the system.
At the beginning of the execution, $T$ is equal to the initial temperature $T_0$ and over the course of the execution, the temperature $T$ decreases.
The way in which $T$ decreases is called the cooling schedule.
Many cooling schedules exist \cite{sa-1, sa-2}.
Most of them operate in rounds of $L$ iterations.
We use $k$ to denote the index of the current round.
$\alpha$ is an additional parameter to steer the speed of the cooling process.
Examples of cooling schedules are:

\begin{itemize}
	\item	Exponential multiplicative cooling: $T = T_0 \cdot \alpha^k$
	\item	Logarithmic multiplicative cooling: $T = \frac{T_0}{1 + \alpha \cdot \log(1+k)}$
	\item	Linear multiplicative cooling: $T = \frac{T_0}{1 + \alpha \cdot k}$
	\item	Quadratic multiplicative cooling: $T = \frac{T_0}{1 + \alpha \cdot k^2}$
\end{itemize}

\input{alg_simulated_annealing.tex}

In our work, we also apply non-monotonic adaptive cooling \cite{sa-nma-cooling} where the temperature obtained by any of the aforementioned cooling schedules is multiplied with a factor $\mu$:

\begin{equation} \label{eq:}
	\mu = \left ( 1 + \frac{C_\text{cur} - C^*}{C_\text{cur}} \right )^\beta
\end{equation}

Here, $C_\text{cur}$ is the cost of the current solution and $C^*$ is the lowest cost that was found over the course of the execution.
$\beta$ is an additional parameter steering the magnitude of the adaptiveness.
The goal of non-monotonic adaptive cooling is to increase the probability of accepting higher-cost solutions in situations where the current solution is far from the best known one (i.e., to escape local optima). 
\Cref{tab:back-sa} summarizes the variables and parameters of the simulated annealing algorithm and \Cref{alg:simulated-annealing} provides its pseudocode.


\input{tab_background_sa}




==> 12_relaxed_constraints.tex <==
\section{Experiments with Relaxed Constraints}
\label{app:relaxed-constraints}

\ps{Introduce experiments with relaxed constraints}

In \Cref{ssec:homo-opt,ssec:hetero-opt}, we use chiplets that are optimized for architectures similar to our baseline, i.e., compute-chiplets have four \gls{phys} and relay-capability while memory-, and IO-chiplets only have a single PHY.
We use these chiplets because architectures like our baseline are the most common today and therefore, such chiplets are most likely to be readily available.
However, this introduces an unfavorable bias against \name~as implementing multiple PHYs and relay-capability in memory- and IO-chiplets would vastly improve the benefits of architectures like the ones found by \name.
Therefore, in this appendix, we repeat all of our experiments with revised chiplets specifications where each compute-, memory-, and IO-chiplet has four \gls{phys} and relay capability.
All remaining parameters are exactly as in the main body of the paper.

\input{fig_app_homo_results}

\input{fig_app_hetero_results}

\input{fig_app_eval_synthetic}

\input{fig_app_eval_trace_full}

\input{fig_app_eval_placements}

\input{fig_app_eval_trace_partial}

\newpage
\Cref{fig:app-homo-results,fig:app-hetero-results} show the results of the optimization process for homogeneous and heterogeneous chiplet shapes, respectively.
We observe that with the revised chiplet specifications, the gap between the three optimization algorithms and the baseline grow considerably. 
The performance differences between the three optimization algorithms themselves are very similar to those in the main body of the paper.


\Cref{fig:app-eval-placements} shows the baseline architectures and the best architectures found by \name.
\Cref{fig:app-eval-synthetic} shows the evaluation on synthetic traffic. 
The benefits of \name~for \gls{c2m}, \gls{c2i}, and \gls{m2i} traffic grew significantly compared to the experiments in the main body of the paper while the disadvantages for \gls{c2c} traffic became less severe.

\Cref{fig:app-eval-trace-full} shows the speedup in average packet latency for the full blackscholes trace. 
We observe that on average, the speedup increased compared to the experiments in the main paper body.
Finally, \Cref{fig:app-eval-trace-partial} shows our results for the simulation of partial trace regions.
Using the revised chiplet specifications, our results are significantly better than with the chiplets tailored to the baseline.
We now reduce the average packet latency for an even larger fraction of the trace-regions, and we reduce it by more, on average, by $18\%$ instead of $8\%$.





==> 13_artifact_description.tex <==
\section{Artifact Description}
\label{app:artifacts}

\paragraph{Requirements}
Hardware: At least 25GB of disk space (mainly for traces) and the capability of running 16 threads in parallel (for the evaluation).
Software: python version 3.11.5 with matplotlib version 3.7.1 and numpy version 1.26.1.

\paragraph{Setup}

Download our framework using the link on the first page.
Download the traces listed in \Cref{tab:eval-traces} from the Netrace website \cite{netrace-traces} and moved them to \textit{./Rapid Chiplet/booksim2/src/netrace/traces/}.
Build BookSim2 by executing \textit{cd ./RapidChiplet/booksim2/src/} and \textit{make}.

\paragraph{Execution}

The script \textit{./reproduce\_placeit\_results.py} reproduces all results. It performs the following steps: 

\begin{enumerate}
	\item	\textbf{Optimization}: Optimize chiplet placements and \gls{ici} topologies for the four architectures. This step reads \textit{./config.py} and stores the results in \textit{./results/}. It is single-threaded and runs for approximately 100 hours.
	\item	\textbf{Evaluation}: Evaluate the optimized architectures using the RapidChiplet \cite{rapidchiplet} toolchain. This step reads the files from \textit{./results/} and traces from \textit{./RapidChiplet/booksim2/ src/netrace/traces/}. It stores evaluation results in \textit{./Rapid Chiplet/results/}. This step spawns up to 16 concurrent threads and runs for approximately 24 hours.
	\item	\textbf{Plotting}: Create all figures in the paper that contain data. This step reads data from \textit{./results/} and \textit{./RapidChiplet/ results/}, and stores the figures in \textit{./plots/}.
\end{enumerate}



==> alg_best_random.tex <==
\begin{algorithm}
\renewcommand{\algorithmcfname}{Alg.}		% Caption is Alg., not Algorithm
\SetAlCapSty{}								% Caption not bold
\hrulefill\\
 best := random\_placement()\\
 \While{Time budget not exceeded}{
  current := random\_placement()\\
  \If{get\_cost(current) $<$ get\_cost(best)}{
   best := current
  }
 }
 \Return{best}\\
\vspace{-0.5em}
\hrulefill
\vspace{0.5em}
\caption{\textbf{(\textsection \ref{app:opt}) The "Best Random" Algorithm.}}
\label{alg:best-random}
\end{algorithm}


==> alg_genetic_algorithm.tex <==
\begin{algorithm}
\renewcommand{\algorithmcfname}{Alg.}		% Caption is Alg., not Algorithm
\SetAlCapSty{}								% Caption not bold
\hrulefill\\
Parameters: $P$, $E$, $T$, $p_m$\\
\vspace{-0.5em}
\hrulefill\\
 pop := list of $P$ randomly generated placements\\
 best := lowest-cost placement from pop\\
 \While{Time budget not exceeded}{
  new\_pop := $E$ lowest-cost placements from pop\\
  \While{length(new\_pop) $<$ $P$}{
   parent1, parent2 := None\\
   \While{parent1 == parent2}{
    tmp1 := $T$ placements of pop selected u.a.r.\\
    parent1 := lowest-cost placement from tmp1\\
    tmp2 := $T$ placements of pop selected u.a.r.\\
    parent2 := lowest-cost placement from tmp2\\
   }
   child = merge(parent1,parent2)\\
   \If{random\_number() $<$ $p_m$}{
    child = mutate(child)
   }
   new\_pop.append(child)
  }
  pop = new\_pop\\
  new\_best := lowest-cost placement from pop\\
  \If{new\_best is better than best}{
    best = new\_best
  }
 }
 \Return{best}\\
\vspace{-0.5em}
\hrulefill
\vspace{0.5em}
\caption{}
\caption{\textbf{(\textsection \ref{app:opt}) The Genetic Algorithm.}}
\label{alg:genetic-algorithm}
\end{algorithm}




==> alg_simulated_annealing.tex <==
\begin{algorithm}
\renewcommand{\algorithmcfname}{Alg.}		% Caption is Alg., not Algorithm
\SetAlCapSty{}								% Caption not bold
\hrulefill\\
Parameters: $T_0$, $L$, $\alpha$, $\beta$\\
\vspace{-0.5em}
\hrulefill\\
 current := random\_placement()\\
 best := current\\
 iteration := 0\\
 \While{Time budget not exceeded}{
  iteration := iteration + 1\\
  new := mutate(current)\\
  $\Delta$ := get\_cost(new) - get\_cost(current)\\
  \eIf{$\Delta < 0$}{
   current = new
  }{
   $k := \lfloor \text{iteration} / L \rfloor$\\
   $T := T_0 / (1 + \alpha \cdot k)$\\
   $\mu :=  \left ( 1 + \frac{\text{get\_cost(current)} - \text{get\_cost(best)}}{\text{get\_cost(current)}} \right )^\beta$\\ 
   $p := \mu \cdot e^{-\Delta / T}$\\
   \If{random\_number() $< p$}{
    current = new 
   }
  }
  \If{get\_cost(current) $<$ get\_cost(best)}{
   best := current
  }
 }
 \Return{best}\\
\vspace{-0.5em}
\hrulefill
\vspace{0.5em}
\caption{\textbf{(\textsection \ref{app:opt}) The Simulated Annealing Algorithm.}}
\label{alg:simulated-annealing}
\end{algorithm}



==> fig_app_eval_placements.tex <==
\begin{figure*}[t]
\centering
\captionsetup{justification=centering}
%
\includegraphics[width=0.85\textwidth]{img/appendix/eval_placements_appendix.pdf}
%
\vspace{-0.5em}
\caption{\textbf{(\textsection \ref{app:relaxed-constraints}) Baseline placements/topologies (top) and optimized placements/topologies found by \name~(bottom).}}
\label{fig:app-eval-placements}
\vspace{-0.5em}
\end{figure*}


==> fig_app_eval_trace_partial.tex <==
\begin{figure*}[t]
\centering
\captionsetup{justification=centering}
\includegraphics[width=0.85\textwidth]{img/appendix/eval_partial_trace_appendix.pdf}
\vspace{-0.5em}
\caption{\textbf{(\textsection \ref{app:relaxed-constraints}) Results for the partial trace regions:} speedup in average packet latency compared to the baseline.\\
We do not show data for the vips trace due to issues with the simulator when simulating that trace.}
\label{fig:app-eval-trace-partial}
\vspace{-1.0em}
\end{figure*}


==> fig_app_hetero_results.tex <==
\begin{figure}[h]
\centering
\captionsetup{justification=centering}
\vspace{-1.0em}
\includegraphics[width=1.0\columnwidth]{img/appendix/hetero_results_appendix.pdf}
%
\caption{\textbf{(\textsection \ref{app:relaxed-constraints}) Results for heterogeneous chiplet shapes.}
We show the evolution of the result over time (left) and the distribution of the final result over 10 repetitions (right).
See \Cref{fig:app-eval-placements} for the placements found by the best algorithm.}
\label{fig:app-hetero-results}
\vspace{-1.75em}
\end{figure}


==> fig_app_homo_results.tex <==
\begin{figure}[h]
\centering
\captionsetup{justification=centering}
\includegraphics[width=1.0\columnwidth]{img/appendix/homo_results_appendix.pdf}
\caption{\textbf{(\textsection \ref{app:relaxed-constraints}) Results for homogeneously shaped chiplets.}
We show the evolution of the result over time (left) and the distribution of the final result over 10 repetitions (right).
See \Cref{fig:app-eval-placements} for the placements found by the best algorithm.}
\label{fig:app-homo-results}
\end{figure}


==> tab_background_ga.tex <==
\begin{table}[h]
\setlength{\tabcolsep}{5pt}
\centering
\captionsetup{justification=centering}
\begin{tabular}{ccl}

\toprule
Parameter	& Domain		& Description
\vspace{-0.3em}\\
\midrule
$P$			& $\mathbb{N}$			& Population size 			\\
$E$			& $\mathbb{N}$, $E<P$ 	& Elitism size 				\\
$T$			& $\mathbb{N}$, $T<P$ 	& Tournament size 			\\
$p_m$		& $[0,1]$				& Mutation probablility		\\
\bottomrule
\end{tabular}
\caption{\textbf{(\textsection \ref{app:opt}) Parameters of the GA.}}
\label{tab:app-ga}
\end{table}



==> tab_background_sa.tex <==
\begin{table}[h]
\setlength{\tabcolsep}{5pt}
\centering
\captionsetup{justification=centering}
\begin{tabular}{ccll}
\toprule
Parameter		& Domain						& Description					& Type
\vspace{-0.3em}\\
\midrule
$p$				& $[0,1]$						& Acceptance probability		& Variable	\\
$\Delta$		& $\mathbb{R}$					& Cost difference				& Variable	\\
$T_0$			& $\mathbb{R^+}$				& Initial temperature			& Parameter	\\
$T$				& $\mathbb{R^+}$, $T \leq T_0$	& Current temperature			& Variable	\\
$L$				& $\mathbb{N}$					& Iterations per round			& Parameter	\\
$k$				& $\mathbb{N}$					& Current round index			& Variable	\\
$\alpha$		& $\mathbb{R^+}$				& Cooling speed					& Parameter	\\
$\mu$			& $\mathbb{R^+}$				& Adaptivity multiplier			& Variable	\\
$C_\text{cur}$	& $\mathbb{R^+}$				& Cost of current solution		& Variable	\\
$C^*$			& $\mathbb{R^+}$				& Cost of best known solution	& Variable	\\
$\beta$			& $\mathbb{R^+}$				& Adaptivity magnitude			& Parameter	\\
\bottomrule
\end{tabular}
\caption{\textbf{(\textsection \ref{app:opt}) Variables and parameters of SA.}}
\label{tab:back-sa}
\end{table}


